Examination Minutes Measurement of Single-Antenna-Element Beamforming

This document shall provide all knowledge gained in conjunction and preparation with the conducted measurements in the antenna measurement chamber of the Institute of Microwave and Wireless Systems (IMW) of the Leibniz University of Hannover (LUH). The measurements have been prepared and conducted by Lukas Grundmann, IMW, and Nils L. Johannsen, Chair of Information and Coding Theory (ICT) of the Christian- Albrechts-University (CAU) of Kiel. This minute shall allow a simpler understanding and quicker reapplication of the required calibrations and system setup for the measurements of further antennas.

==> tikz/BlockDiagramAntennaPattern.tex <==
% From https://tex.stackexchange.com/questions/200235/is-there-a-predefined-bandpass-filter-block-in-tikz

\newcommand{\cross}[1] 
{  % #1 = name , 
\draw[thick] (#1) circle (12pt);
\draw[rotate=45,line width=0.5pt]   (#1)  +(0,-12pt) -- +(0,12pt);
\draw[rotate=-45,line width=0.5pt]  (#1)  +(0,-12pt) -- +(0,12pt);
}

\newcommand{\BPF}[2] 
{  % #1 = name , #2 = rotation angle
\begin{inks}[transform shape,rotate=#2]
\draw[thick] (#1)node[](a){} +(-12pt,-12pt) rectangle +(12pt,12pt);
\draw (a) +(-8pt,0) to[bend left] +(0,0) edge[bend right] +(8pt,0);
\draw ([yshift=5pt]a) +(-8pt,0) to[bend left] +(0,0) to[bend right] +(8pt,0);
\draw ([yshift=-5pt]a) +(-8pt,0) to[bend left] +(0,0) edge[bend right] +(8pt,0);
\draw[rotate=20] ([yshift=5pt]a) +(-4pt,0) -- +(7pt,0);
\draw[rotate=20] ([yshift=-5pt]a) +(-7pt,0) -- +(4pt,0);
\end{scope}
}

\tikzset{ar/.style={-latex,shorten >=-1pt, shorten <=-1pt}}


\begin{circuitikz}
\path (4,0) node[above=2pt]() {LO} to[sV]node[pos=0,inner sep=0pt](b){} (4,2);
\draw (0,3) node[buffer,scale=0.8](buf){}
node[above =0.8 cm]{LNA};
\path (1,3) to[sV,color=white,name=bp]
node[pos=0,inner sep=0pt](d){}
node[above left=0.8cm and 0.2cm]{BPF} (3,3);
\BPF{bp}{0}
\path (4,2) to[sV,color=white,name=M1]node[midway,above=0.1cm]{Mixer}(4,4);
\cross{M1}
\draw[] (-1,3) node [antenna,xscale=-1] (A) {}--(buf.in);
\draw[ar] (bp)--(M1);
\draw[ar] (buf.out)--(bp);
\draw[ar] (b)--(M1);
\draw[ar] (M1) -- +(2,0);
%\draw (0,6) node[buffer,scale=1.0](buf){}
\draw (3,0) to[R, i>^=$I_A$, l=$R_A$] (3,3);

\end{circuitikz}
